Using Name Confusion to Enhance Security

We introduce a novel concept, called Name Confusion, and demonstrate how it can be employed to thwart multiple classes of code-reuse attacks. By building upon Name Confusion, we derive Phantom Name System (PNS): a security protocol that provides multiple names (addresses) to program instructions. Unlike the conventional model of virtual memory with a one-to-one mapping between instructions and virtual memory addresses, PNS creates N mappings for the same instruction, and randomly switches between them at runtime. PNS achieves fast randomization, at the granularity of basic blocks, which mitigates a class of attacks known as (just-in-time) code-reuse. If an attacker uses a memory safety-related vulnerability to cause any of the instruction addresses to be different from the one chosen during a fetch, the exploited program will crash. We quantitatively evaluate how PNS mitigates real-world code-reuse attacks by reducing the success probability of typical exploits to approximately $10^{-12}$. We implement PNS and validate it by running SPEC CPU2017 benchmark suite. We further verify its practicality by adding it to a RISC-V core on an FPGA. Lastly, PNS is mainly designed for resource constrained (wimpy) devices and has negligible performance overhead, compared to commercially-available, state-of-the-art, hardware-based protections.

==> motivation.tex <==
\begin {comment}
\section{Motivation}\label{sec:motivation}
In this paper, we examine CRA defenses in the context of resources constrained architectures. To understand the need for novel techniques in this area, in this section, we revisit techniques that are used to protect high-end systems and discuss their applicability in the context of mitigating CRAs.

\fakesubsub{\EPREx{}.}
The idea of \EPREx{}, described in
Section~\ref{sub:isomeron}, was first introduced by Davi \emph{et
al.}~\cite{isomeron2015}. Their work was realized purely in software, and, as a
result, has a number of (performance) limitations.
\begin{enumerate}[nosep]
	\item It leverages dynamic binary instrumentation
		(DBI)~\cite{Nethercote2004}: to: (a)~instrument all
		\texttt{call}, \texttt{ret}, and \texttt{jmp} instructions
		executed by the program; and (b)~modify/insert (new) code into
		the instruction stream. The overheads of their instrumentation
		is in addition to those of the DBI framework itself. DBI
		framework overheads can vary anywhere from~$5\%$ to~$50\%$
		depending on the complexity of the program being
		instrumented~\cite{dbiperf2008}.

  \item Isomeron increases the memory pressure on the system, as it
		requires two duplicate copies of the code to be loaded into the
		program's address space. As a result, this adds more TLB and
		I-Cache misses.
	\item The random diversifier wreaks havoc on the effectiveness of
		branch prediction units in hardware. This results in low
		prediction accuracy, amounting to wasted execution in
		out-of-order processors.
\end{enumerate}


There are two fundamental sources of overhead with Isomeron, and
an artefactual overhead.  First, Isomeron increases the memory
pressure on the system, as it requires two duplicate copies of the
code to be loaded into the program's address space.  As a result,
this adds more TLB and I-Cache misses.  Second, the random diversifier
wreaks havoc on the effectiveness of branch prediction units in
hardware.  This results in low prediction accuracy, amounting to
wasted execution in out-of-order processors.  Finally, the authors
of the original paper proposed using Dynamic Binary Instrumentation
to create variants and hook on to control-transfer instructions.
These overheads alone can be close to ~5\% to ~50\%~\cite{dbiperf2008}
depending on the complexity of the instrumented program.  The overall
overheads of the software Isomeron scheme are close to 400\%.
Crucially, the above are only exacerbated in resource constrained
settings, such as IoT devices, as the majority of these platforms
use much smaller address spaces and simpler CPUs.
\end{comment}







